Evaluating the Values of Sources in Transfer Learning

Transfer learning that adapts a model trained on data-rich sources to low-resource targets has been widely applied in natural language processing (NLP). However, when training a transfer model over multiple sources, not every source is equally useful for the target. To better transfer a model, it is essential to understand the values of the sources. In this paper, we develop SEAL-Shap, an efficient source valuation framework for quantifying the usefulness of the sources (e.g., domains/languages) in transfer learning based on the Shapley value method. Experiments and comprehensive analyses on both cross-domain and cross-lingual transfers demonstrate that our framework is not only effective in choosing useful transfer sources but also the source values match the intuitive source-target similarity.

==> ethics.tex <==
\section{Ethics/Broader Impact Statement}

In any systems, the end performance depends on a large number of factors. Factors may have different correlation or impact to the end result. Identifying the useful components can, therefore, enhance the end results  in many aspects. However, measuring the significance of a component is burdensome when it associates a lot computation.  A reduced overhead and resource utilization in identifying the positive and negative impact factors can therefore bring about a significant  well beings to the society. 
% Imagine a case where we have the medical history of a number of patients of a rear disease. The history includes several behaviors of the patients. And it may be possible that a few of these behavioral actions have correlation with the disease. However, to identify them, we need to know their relevance with the disease.
In this paper, we develop an efficient source valuation method that estimates usefulness of a source to the corresponding target. This work can be applied to many AI system to evaluate the value of different factors for a target task. Starting from agriculture, medicals, education systems to find the bugs in a software.  


Another benefit of our approach is that it  can make models explainable to some extent. We present evidences that our source values are meaningful and it captures different relation information. Hence this tool can be used for reasoning and model interpretability. Human can understand why the model is predicting that there is high chance of security breach, why the state may face an inflation and so on.  


However, among the negative aspects of our approach is that it is still expensive when for a set of sources the number target task is very limited. For example, in the application of agriculture, we need to find what weather is good for producing only one harvest then the computation gain is very limited.  Also it needs a lots of tuning and may be sub-optimal. In case of precise prediction, this approximation may be wrong or less effective and we should be cautious about that.  
